Morphological Matrices as a Tool for Crowdsourced Ideation

Designing a novel product is a difficult task not well suited for non-expert crowd workers. In this work-in-progress paper, we first motivate why the design of persuasive products is an interesting context for studying creativity and the creative leap. We then present a pilot study on the crowdsourced design of persuasive products. The pilot study motivated our subsequent feasibility study on the use of morphological matrices as a tool for crowdsourced ideation and product design. Given the morphological matrix, workers were able to come up with valid and significantly more relevant ideas for novel persuasive products.

==> HCOMP21-WIP_ Morphological Matrix Ideation (2021-09-10)/TAB-PRINCIPLES.tex <==

\begin{table*}[t]
\centering
% \scriptsize
% \begin{tabularx}{\textwidth}{
%     >{\hsize=1.5\hsize\raggedright\arraybackslash}X
%     |
%     >{\hsize=.8\hsize\raggedright\arraybackslash}X
%     |
%     >{\hsize=.8\hsize\raggedright\arraybackslash}X
%     |
%     >{\hsize=.8\hsize\raggedright\arraybackslash}X
%     |
%     >{\hsize=.8\hsize\raggedright\arraybackslash}X
%     |
%     >{\hsize=.8\hsize\raggedright\arraybackslash}X
%     |
%     >{\hsize=.8\hsize\raggedright\arraybackslash}X
%     |
%     >{\hsize=.8\hsize\raggedright\arraybackslash}X
% }
%     \textbf{Category}
% &
% \multicolumn{7}{c}{
%     \textbf{Design options (principles)}
% }
% \\
% \hline
% \raggedright
% \textbf{Primary Task Support} &
% Reduction &
% Tunneling &
% Tailoring &
% Personalization &
% Self-monitoring &
% Simulation &
% Rehearsal
% \\
% \hline
% \raggedright
% \textbf{Dialogue Support} &
% Praise &
% Rewards &
% Reminders &
% Suggestion &
% Similarity &
% Liking &
% Social role
% \\
% \hline
% \raggedright
% \textbf{System Credibility Support} &
% Trustworthiness &
% Expertise &
% Surface \newline credibility & 
% Real-world feel &
% Authority &
% Third-party endorsements & 
% Verifiability
% \\
% \hline
% \raggedright
% \textbf{Social support} &
% Social learning &
% Social comparison & 
% Normative \newline influence & 
% Social facilitation  &
% Cooperation &
% Competition &
% Recognition
% \\
% \hline
% \end{tabularx}
%}
% \includegraphics[width=0.98\textwidth]{tabledraft.png}% Reduce the figure size so that it is slightly narrower 
\input{TROUBLEMAKERS}
\caption{Design principles of ``pleasurable troublemakers'' \cite{Laschke2014}
% by \citet{design-principles} arranged as a morphological matrix with two exemplary sets of combinations highlighted. For each of the design principles, \citet{design-principles} provide descriptions which were used as instructions for crowdsourcing tasks in the feasibility study.
}%
\label{tab:morphologicalbox}%
\end{table*}%






==> HCOMP21-WIP_ Morphological Matrix Ideation (2021-09-10)/TAB-TROUBLEMAKERS.tex <==

\begin{table*}[t]
\centering
\scriptsize
\begin{tabularx}{.95\textwidth}{
    >{\hsize=.4\hsize\raggedright\arraybackslash}X
    |
    >{\hsize=1.15\hsize\raggedright\arraybackslash}X
    >{\hsize=1.15\hsize\raggedright\arraybackslash}X
    >{\hsize=1.15\hsize\raggedright\arraybackslash}X
    >{\hsize=1.15\hsize\raggedright\arraybackslash}X
}
\hline
\raggedright
    Principle &
    \textit{Situatedness} &
    \textit{Alternative Choice} &
    \textit{Freedom} &
    \textit{Meaning-making}
\\
\hline
    Description of principle
    &
    The system is situated in  a  moment  of  choice. The system accomplishes its goal by creating ``friction'' based on knowledge of the situation. 
    &
    The system expands the available choices in order to provide an alternative  action  in  line  with  a desirable course of action.
    &
    The system % alters the moment of choice, but
    does not pressure or threaten the user into taking an action. % nor make it simpler for the user.
     Users have the freedom to ignore the system's suggested course of action and have a choice to cheat the system.
    &
    The system encourages the user to reflect on their choice. While the system can be cheated, the user would cheat on their own goals.
\\
\hline
    Example &
    A keyholder drops a bicycle  key to the floor if a user reaches for the car key. This motivates the user to use the bicycle more often.
    &
    An elevator stops one story short of the intended one. The user therefore is motivated to be more physically active and walk the remaining flight of stairs.
    &
    A clothing holder drops sport clothing to the floor if it is not used. Users still have the choice to ignore the suggested course of action.
    &
    A calendar drops agenda items when the user procrastinates, but one can add them again, even when not completed.
\\
\hline
\end{tabularx}
\caption{Design principles of ``pleasurable troublemakers'' \cite{Laschke2014}.
Descriptions and examples adapted from \citet{3461778.3462079.pdf}.
% by \citet{design-principles} arranged as a morphological matrix with two exemplary sets of combinations highlighted. For each of the design principles, \citet{design-principles} provide descriptions which were used as instructions for crowdsourcing tasks in the feasibility study.
}%
\label{tab:morphologicalbox}%
\end{table*}%






==> TAB-PRINCIPLES.tex <==

\begin{table*}[t]
\centering
% \scriptsize
% \begin{tabularx}{\textwidth}{
%     >{\hsize=1.5\hsize\raggedright\arraybackslash}X
%     |
%     >{\hsize=.8\hsize\raggedright\arraybackslash}X
%     |
%     >{\hsize=.8\hsize\raggedright\arraybackslash}X
%     |
%     >{\hsize=.8\hsize\raggedright\arraybackslash}X
%     |
%     >{\hsize=.8\hsize\raggedright\arraybackslash}X
%     |
%     >{\hsize=.8\hsize\raggedright\arraybackslash}X
%     |
%     >{\hsize=.8\hsize\raggedright\arraybackslash}X
%     |
%     >{\hsize=.8\hsize\raggedright\arraybackslash}X
% }
%     \textbf{Category}
% &
% \multicolumn{7}{c}{
%     \textbf{Design options (principles)}
% }
% \\
% \hline
% \raggedright
% \textbf{Primary Task Support} &
% Reduction &
% Tunneling &
% Tailoring &
% Personalization &
% Self-monitoring &
% Simulation &
% Rehearsal
% \\
% \hline
% \raggedright
% \textbf{Dialogue Support} &
% Praise &
% Rewards &
% Reminders &
% Suggestion &
% Similarity &
% Liking &
% Social role
% \\
% \hline
% \raggedright
% \textbf{System Credibility Support} &
% Trustworthiness &
% Expertise &
% Surface \newline credibility & 
% Real-world feel &
% Authority &
% Third-party endorsements & 
% Verifiability
% \\
% \hline
% \raggedright
% \textbf{Social support} &
% Social learning &
% Social comparison & 
% Normative \newline influence & 
% Social facilitation  &
% Cooperation &
% Competition &
% Recognition
% \\
% \hline
% \end{tabularx}
%}
% \includegraphics[width=0.98\textwidth]{tabledraft.png}% Reduce the figure size so that it is slightly narrower 
\input{TROUBLEMAKERS}
\caption{Design principles of ``pleasurable troublemakers'' \cite{Laschke2014}
% by \citet{design-principles} arranged as a morphological matrix with two exemplary sets of combinations highlighted. For each of the design principles, \citet{design-principles} provide descriptions which were used as instructions for crowdsourcing tasks in the feasibility study.
}%
\label{tab:morphologicalbox}%
\end{table*}%






==> TAB-TROUBLEMAKERS.tex <==

\begin{table*}[t]
\centering
\scriptsize
\begin{tabularx}{.95\textwidth}{
    >{\hsize=.4\hsize\raggedright\arraybackslash}X
    |
    >{\hsize=1.15\hsize\raggedright\arraybackslash}X
    >{\hsize=1.15\hsize\raggedright\arraybackslash}X
    >{\hsize=1.15\hsize\raggedright\arraybackslash}X
    >{\hsize=1.15\hsize\raggedright\arraybackslash}X
}
\hline
\raggedright
    Principle &
    \textit{Situatedness} &
    \textit{Alternative Choice} &
    \textit{Freedom} &
    \textit{Meaning-making}
\\
\hline
    Description of principle
    &
    The system is situated in  a  moment  of  choice. The system accomplishes its goal by creating ``friction'' based on knowledge of the situation. 
    &
    The system expands the available choices in order to provide an alternative  action  in  line  with  a desirable course of action.
    &
    The system % alters the moment of choice, but
    does not pressure or threaten the user into taking an action. % nor make it simpler for the user.
     Users have the freedom to ignore the system's suggested course of action and have a choice to cheat the system.
    &
    The system encourages the user to reflect on their choice. While the system can be cheated, the user would cheat on their own goals.
\\
\hline
    Example &
    A keyholder drops a bicycle  key to the floor if a user reaches for the car key. This motivates the user to use the bicycle more often.
    &
    An elevator stops one story short of the intended one. The user therefore is motivated to be more physically active and walk the remaining flight of stairs.
    &
    A clothing holder drops sport clothing to the floor if it is not used. Users still have the choice to ignore the suggested course of action.
    &
    A calendar drops agenda items when the user procrastinates, but one can add them again, even when not completed.
\\
\hline
\end{tabularx}
\caption{Design principles of ``pleasurable troublemakers'' \cite{Laschke2014}.
Descriptions and examples adapted from \citet{3461778.3462079.pdf}.
% by \citet{design-principles} arranged as a morphological matrix with two exemplary sets of combinations highlighted. For each of the design principles, \citet{design-principles} provide descriptions which were used as instructions for crowdsourcing tasks in the feasibility study.
}%
\label{tab:morphologicalbox}%
\end{table*}%





